Design and Evaluation of Alternate Enumeration Techniques for Subset Sum Problem

The subset sum problem, also referred as SSP, is a NP-Hard computational problem. SSP has its applications in broad domains like cryptography, number theory, operation research and complexity theory. The most famous algorithm for solving SSP is Backtracking Algorithm which has exponential time complexity. Therefore, our goal is to design and develop better alternate enumeration techniques for faster generation of SSP solutions. Given the set of first n natural numbers which is denoted by Xn and a target sum S, we propose various alternate enumeration techniques which find all the subsets of Xn that add up to sum S. In this paper, we present the mathematics behind this exponential problem. We analyze the distribution of power set of Xn and present formulas which show definite patterns and relations among these subsets. We introduce three major distributions for power set of Xn: Sum Distribution, Length-Sum Distribution and Element Distribution. These distributions are prepossessing procedures for various alternate enumeration techniques for solving SSP. We propose novel algorithms: Subset Generation using Sum Distribution, Subset Generation using Length-Sum Distribution, Basic Bucket Algorithm, Maximum and Minimum Frequency Driven Bucket Algorithms and Local Search using Maximal and Minimal Subsets for enumerating SSP. We compare the performance of these approaches against the traditional backtracking algorithm. The efficiency and effectiveness of these algorithms are presented with the help of these experimental results. Furthermore, we studied the over solution set of subsets generated by various algorithms to get the complete solution for subset sum problem. Finally, we present a conjecture about upper bound on the number of subsets that has to be enumerated to get all solutions for Subset Sum Problem.

==> pgfsubpic.tex <==
%    pgfsubpic.tex
%    Version 1.1, 25 Dec 2009

%    Copyright 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.1:
% - the ability to save a subpicture in local variables
% - nodes in subpictures are tracked if the subpicture is placed with arbitrary transforms
% - new \pgffitsubpicture macro to transform a subpicture (preserving aspect) to fit in a desired box

\newdimen\pgf@subpicminx
\newdimen\pgf@subpicminy
\newdimen\pgf@subpicmaxx
\newdimen\pgf@subpicmaxy

% Special virtual node for current subpicture's bounding box
\expandafter\def\csname pgf@sh@ns@current subpicture\endcsname{rectangle}
\expandafter\def\csname pgf@sh@np@current subpicture\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@subpicminx}{\pgf@subpicminy}}%
  \def\northeast{\pgfqpoint{\pgf@subpicmaxx}{\pgf@subpicmaxy}}%
}
\expandafter\def\csname pgf@sh@nt@current subpicture\endcsname{{\pgf@pt@aa}{\pgf@pt@ab}{\pgf@pt@ba}{\pgf@pt@bb}{\the\pgf@pt@x}{\the\pgf@pt@y}} % the transformation at invocation time
\expandafter\def\csname pgf@sh@pi@current subpicture\endcsname{\pgfpictureid}

% Create a pgfpicture inside an hbox for delayed placement
\def\pgfsubpicture{%
\expandafter\global\expandafter\setbox\pgf@hbox=\hbox\bgroup
\pgfinterruptpicture
\pgfpicture
\relax % not sure why. otherwise a curly brace immediately after causes an error
}

\def\endpgfsubpicture{
\global\pgf@subpicminx=\pgf@picminx
\global\pgf@subpicminy=\pgf@picminy
\global\pgf@subpicmaxx=\pgf@picmaxx
\global\pgf@subpicmaxy=\pgf@picmaxy
\global\edef\subpictureid{\pgfpictureid}%
\pgfsetbaseline{\pgf@picminy}%
\endpgfpicture%
\endpgfinterruptpicture%
\egroup
}

% Allocate registers for saving a subpicture. #1 is text, not a control sequence.
\def\pgfnewsubpicture#1{%
\expandafter\newbox\csname pgf@subpic@hbox@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@minx@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@miny@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@maxx@#1\endcsname
\expandafter\newdimen\csname pgf@subpic@maxy@#1\endcsname
}

% saved subpictures are local to the current group
\def\pgfsavesubpicture#1{%
\expandafter\setbox\csname pgf@subpic@hbox@#1\endcsname\box\pgf@hbox
\csname pgf@subpic@minx@#1\endcsname\pgf@subpicminx
\csname pgf@subpic@miny@#1\endcsname\pgf@subpicminy
\csname pgf@subpic@maxx@#1\endcsname\pgf@subpicmaxx
\csname pgf@subpic@maxy@#1\endcsname\pgf@subpicmaxy
\expandafter\edef\csname pgf@subpic@id@#1\endcsname{\subpictureid}%
}

% place current subpicture into named subpicture
\def\pgfmergesubpicture#1{%
\begin{pgfsubpicture}
% place current subpicture
\pgfplacesubpicture
% override containing picture
\expandafter\xdef\csname pgf@sh@pi@\subpictureid\endcsname{\csname pgf@subpic@id@#1\endcsname}%
% copy contents of #1
\pgfrestoresubpicture{#1}
\pgflowlevelobj{\pgftransformshift{\pgfqpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}}{\pgfqbox\pgf@hbox}
\pgfpathrectanglecorners{\pgfqpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}{\pgfqpoint{\the\pgf@subpicmaxx}{\the\pgf@subpicmaxy}}%
\pgfusepath{use as bounding box}%
%
\end{pgfsubpicture}
\expandafter\setbox\csname pgf@subpic@hbox@#1\endcsname\box\pgf@hbox
\csname pgf@subpic@minx@#1\endcsname\pgf@subpicminx
\csname pgf@subpic@miny@#1\endcsname\pgf@subpicminy
\csname pgf@subpic@maxx@#1\endcsname\pgf@subpicmaxx
\csname pgf@subpic@maxy@#1\endcsname\pgf@subpicmaxy
% but don't save the new picture id, keep the existing one
}

\def\pgfrestoresubpicture#1{%
\edef\act{\global\noexpand\setbox\pgf@hbox\noexpand\box\csname pgf@subpic@hbox@#1\endcsname}\act
\expandafter\global\expandafter\pgf@subpicminx\csname pgf@subpic@minx@#1\endcsname
\expandafter\global\expandafter\pgf@subpicminy\csname pgf@subpic@miny@#1\endcsname
\expandafter\global\expandafter\pgf@subpicmaxx\csname pgf@subpic@maxx@#1\endcsname
\expandafter\global\expandafter\pgf@subpicmaxy\csname pgf@subpic@maxy@#1\endcsname
\xdef\subpictureid{\csname pgf@subpic@id@#1\endcsname}%
}

% Place a previously-created subpicture, lining up its origin with the current origin
\def\pgfplacesubpicture{
\pgfscope
% expand current bounding box to accommodate subpicture
\pgfpathrectanglecorners{\pgfqpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}{\pgfqpoint{\the\pgf@subpicmaxx}{\the\pgf@subpicmaxy}}%
\pgfusepath{use as bounding box}%
%
% make the subpicture a node in the containing picture
\expandafter\gdef\csname pgf@sh@ns@\subpictureid\endcsname{rectangle}%
\expandafter\xdef\csname pgf@sh@np@\subpictureid\endcsname{%
  \noexpand\def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}%
  \noexpand\def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@subpicmaxx}{\the\pgf@subpicmaxy}}%
}%
\pgfgettransform\pgf@temp
\expandafter\xdef\csname pgf@sh@nt@\subpictureid\endcsname{\pgf@temp}%
\expandafter\xdef\csname pgf@sh@pi@\subpictureid\endcsname{\pgfpictureid}%
%
% align origin of subpicture with origin
\pgftransformshift{\pgfqpoint{\the\pgf@subpicminx}{\the\pgf@subpicminy}}%
\pgfqboxsynced{\pgf@hbox}%
\endpgfscope
}

% Hook onto existing macro \pgf@shape@interpictureshift.
% This is called whenever we look up an anchor of a node.
% This hook recursively checks to see if the node's picture
% is a subpicture of another, and if so, adjusts its position accordingly.

% This is slow. It makes drawing trees O(n^2) in the depth of the tree.
% The alternative is to store, for each picture, a list of the nodes
% inside it. But this way doesn't require us to hijack \pgfnode, and
% is robust to re-placement of a subpicture. A compromise would be
% to store, for each picture, a list of the *subpictures* inside it.

\let\orig@pgf@shape@interpictureshift\pgf@shape@interpictureshift
\def\unwind@subpic#1{%
% is #1 the current picture?
\edef\subpicid{#1}%
\ifx\subpicid\pgfpictureid
% yes, we're done
\else
% does #1 have a parent picture?
\expandafter\ifx\csname pgf@sh@pi@#1\endcsname\relax
% no, the original node was not inside the current picture
\fallback
\else
% yes, apply transform and move up to parent picture
{%
  \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
  \pgf@pos@transform{\pgf@x}{\pgf@y}%
  \global\pgf@x=\pgf@x
  \global\pgf@y=\pgf@y
}%
\unwind@subpic{\csname pgf@sh@pi@#1\endcsname}%
\fi
\fi
}
\def\pgf@shape@interpictureshift#1{%
\edef\fallback{\pgf@x=\the\pgf@x\pgf@y=\the\pgf@y\noexpand\orig@pgf@shape@interpictureshift{#1}}%
\unwind@subpic{\csname pgf@sh@pi@#1\endcsname}%
}

% \pgffitsubpicture{sw}{ne}
% Make the subpicture fit in the rectangle from sw to ne, preserving its aspect ratio.
\def\pgffitsubpicture#1#2{%
% current size
\pgfpointdiff{\pgfpointanchor{current subpicture}{south west}}{\pgfpointanchor{current subpicture}{north east}}%
\pgf@xa=\pgf@x \pgf@ya=\pgf@y
% desired size
\pgf@process{\pgfpointdiff{#1}{#2}}%
\pgf@xb=\pgf@x \pgf@yb=\pgf@y
\pgfmathparse{min(\pgf@xb/\pgf@xa,\pgf@yb/\pgf@ya)}%
\pgfmathparse{min(1,\pgfmathresult)}%
\pgftransformscale{\pgfmathresult}%
%
% current position
\pgfpointanchor{current subpicture}{center}%
\pgf@xa=\pgf@x \pgf@ya=\pgf@y
% desired position
% we scaled transform, so apply reverse scaling to argument
\pgfmathparse{1/\pgfmathresult}%
\pgf@process{\pgfpointscale{\pgfmathresult}{\pgfpointlineattime{0.5}{#1}{#2}}}%
\pgf@xb=\pgf@x \pgf@yb=\pgf@y
\pgfpointdiff{\pgfpoint{\pgf@xa}{\pgf@ya}}{\pgfpoint{\pgf@xb}{\pgf@yb}}%
\pgftransformshift{\pgfpoint{\pgf@x}{\pgf@y}}%
}

% utility functions -- not currently used

\def\pgfnodedelete#1{%
\expandafter\global\expandafter\let\csname pgf@sh@ns@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@np@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@nt@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@pi@#1\endcsname\relax
\expandafter\global\expandafter\let\csname pgf@sh@ma@#1\endcsname\relax
}

\def\pgfnodeifexists#1#2#3{%
\expandafter\ifx\csname pgf@sh@ns@#1\endcsname\relax#3\else#2\fi
}



==> pgftree.tex <==
%    pgftree.tex
%    Version 1.2, 20 Apr 2012

%    Copyright 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.2:
% - level-specific styles (thanks to Andrew Stacey)

% New in version 1.1:
% - major restructuring to not do arbitrary nesting of subpicture environments
% - sideways trees

% To do:
% - trees with all leaves at same level
% - if \nodename does not exist as desired, wrap inside a rectangle node
% - don't use pgfsubpic internals

\newdimen\levelsep \levelsep=30pt
\newdimen\subtreesep \subtreesep=2pt
\newdimen\smuggle@levelsep
\newdimen\smuggle@subtreesep
\newdimen\this@levelsep
\newdimen\this@subtreesep

\def\leveldirection{down}
\def\siblingdirection{right}

% definitions of growing directions
\def\pgftree@levelshift{\csname pgftree@levelshift@\leveldirection\endcsname}
\def\pgftree@parentanchor{\csname pgftree@parentanchor@\leveldirection\endcsname}
\def\pgftree@childanchor{\csname pgftree@childanchor@\leveldirection\endcsname}
% these assume that the current subpicture is the child
\def\pgftree@presiblingshift{\csname pgftree@presiblingshift@\siblingdirection\endcsname}
\def\pgftree@postsiblingshift{\csname pgftree@postsiblingshift@\siblingdirection\endcsname}

\def\pgftree@levelshift@down{\pgfpoint{0}{-\levelsep}}
\def\pgftree@parentanchor@down{south}
\def\pgftree@childanchor@down{north}

\def\pgftree@levelshift@up{\pgfpoint{0}{\levelsep}}
\def\pgftree@parentanchor@up{north}
\def\pgftree@childanchor@up{south}

\def\pgftree@levelshift@right{\pgfpoint{\levelsep}{0}}
\def\pgftree@parentanchor@right{east}
\def\pgftree@childanchor@right{west}

\def\pgftree@levelshift@left{\pgfpoint{-\levelsep}{0}}
\def\pgftree@parentanchor@left{west}
\def\pgftree@childanchor@left{east}

\def\pgftree@presiblingshift@right{\pgf@process{\pgf@x-\pgf@subpicminx \advance\pgf@x\subtreesep \pgf@y 0pt}}
\def\pgftree@postsiblingshift@right{\pgf@process{\pgf@x\pgf@subpicmaxx \pgf@y 0pt}}

\def\pgftree@presiblingshift@left{\pgf@process{\pgf@x-\pgf@subpicmaxx \advance\pgf@x-\subtreesep \pgf@y 0pt}}
\def\pgftree@postsiblingshift@left{\pgf@process{\pgf@x\pgf@subpicminx \pgf@y 0pt}}

\def\pgftree@presiblingshift@up{\pgf@process{\pgf@x 0pt \pgf@y-\pgf@subpicminy \advance\pgf@y\subtreesep}}
\def\pgftree@postsiblingshift@up{\pgf@process{\pgf@x 0pt \pgf@y\pgf@subpicmaxy}}

\def\pgftree@presiblingshift@down{\pgf@process{\pgf@x 0pt \pgf@y-\pgf@subpicmaxy \advance\pgf@y-\subtreesep}}
\def\pgftree@postsiblingshift@down{\pgf@process{\pgf@x 0pt \pgf@y\pgf@subpicminy}}

% for convenience if you are using \pgftree directly
\def\drawnode#1{\pgfnode{rectangle}{base}{#1}{\nodename}{\pgfusepath{discard}}}
\def\drawedge{%
\pgfpathmoveto{\pgfpointanchor{\parentnodename}{\pgftree@parentanchor}}%
\pgfpathlineto{\pgfpointanchor{\nodename}{\pgftree@childanchor}}%
\pgfusepath{stroke}}

% local variables that we need to assign to inside a \pgfforeach
\newdimen\pgftree@childx
\newdimen\pgftree@savechildx
\newdimen\pgftree@childy
\newdimen\pgftree@savechildy
\newcount\pgftree@childi
\newcount\pgftree@savechildi
\newcount\pgftree@level
\newdimen\pgftree@depth

%%% \pgftree{subtree}

\def\pgftree#1{%
\def\nodename{r}%
\pgftree@level=0\relax
\pgftree@depth=0pt\relax
#1%
\pgfplacesubpicture
}

%%% \pgfsubtree{root}{subtrees}
% The first argument draws the root node using PGF/TikZ commands.
% The node must be named \nodename.

% The second argument is a sequence of 3n tokens.
% Token 3n-2 draws the nth edge. It should draw an edge from \parentnodename to \nodename.
% Token 3n-1 is a hook that can change \levelsep or \subtreesep for child n only.
% Token 3n draws the nth subtree. Its root must be named \nodename.

\pgfnewsubpicture{children}
\newdimen\pgftree@lastchildx
\newdimen\pgftree@lastchildy

\def\pgfsubtree#1#2{%
\let\parentnodename\nodename
\pgftree@savechildx=\pgftree@childx
\pgftree@savechildy=\pgftree@childy
\pgftree@savechildi=\pgftree@childi
% Build subpicture with all the children and their subtrees
{\pgftree@childx=0pt%
\pgftree@childy=0pt%
\pgftree@childi=0%
\process@children #2}%
\begin{pgfsubpicture}%
% Create node
#1%
\ifnum\pgftree@childi>0%
% Place children
{% center so that parent is midway between origins of first and last children
\pgftransformshift{\pgfpointscale{-0.5}{\pgfqpoint{\the\pgftree@childx}{\the\pgftree@childy}}}%
\pgfplacesubpicture}%
% Draw the edges
{\pgftree@childi=0%
\process@edges #2}%
\fi
\end{pgfsubpicture}%
\global\pgftree@childi=\pgftree@savechildi
\global\pgftree@childx=\pgftree@savechildx
\global\pgftree@childy=\pgftree@savechildy
}

\def\process@children{%
\pgfutil@ifnextchar\egroup
{% No more children, step back to origin of last child
\global\pgftree@childx\pgftree@lastchildx
\global\pgftree@childy\pgftree@lastchildy
\global\pgftree@childi\pgftree@childi
\ifnum\pgftree@childi>0%
\pgfrestoresubpicture{children}% pass children back to caller
\fi
}%
{\@process@children}%
}
\def\@process@children#1#2#3{% 
% #1 is the edge, #2 is the hook, #3 is the child
{% call hook to get \levelsep and \subtreesep
% and put them in \this@levelsep and \this@subtreesep
% to hide them from descendants
#2%
\global\smuggle@levelsep\levelsep
\global\smuggle@subtreesep\subtreesep}%
\this@levelsep\smuggle@levelsep
\this@subtreesep\smuggle@subtreesep
% Build the current child
{\edef\nodename{\parentnodename-\the\pgftree@childi}%
\advance\pgftree@level by 1\relax
\advance\pgftree@depth by \this@levelsep
#3}%
\begin{pgfsubpicture}%
% Place current child
{%
% The \levelsep and \subtreesep set in #2 apply only here
\levelsep\this@levelsep
\subtreesep\this@subtreesep
\ifnum\pgftree@childi>0% the first child is always at 0
\pgftree@presiblingshift \global\advance\pgftree@childx\pgf@x \global\advance\pgftree@childy\pgf@y
\fi
\pgftransformshift{\pgftree@levelshift}%
\pgftransformshift{\pgfqpoint{\the\pgftree@childx}{\the\pgftree@childy}}%
\pgfplacesubpicture
\global\pgftree@lastchildx\pgftree@childx
\global\pgftree@lastchildy\pgftree@childy
\pgftree@postsiblingshift \global\advance\pgftree@childx\pgf@x \global\advance\pgftree@childy\pgf@y
}%
% Save the augmented row of children back into "children"
\end{pgfsubpicture}
\ifnum\pgftree@childi>0%
\pgfmergesubpicture{children}
\else
\pgfsavesubpicture{children}%
\fi
\advance\pgftree@childi by 1%
\process@children
}

\def\process@edges{%
\pgfutil@ifnextchar\egroup
{}%
{\@process@edges}%
}
\def\@process@edges#1#2#3{%
\edef\nodename{\parentnodename-\the\pgftree@childi}%
#1%
\advance\pgftree@childi by 1%
\process@edges
}

\def\subtreeof#1{%
% the subpicture which contains a node also contains exactly its subtree
\csname pgf@sh@pi@#1\endcsname
}


==> tikz-qtree.tex <==
%    tikz-qtree.tex
%    Version 1.2, 20 Apr 2012

%    Copyright (C) 2002, 2009 by David Chiang

%    This program is free software; you can redistribute it and/or modify
%    it under the terms of the GNU General Public License as published by
%    the Free Software Foundation; either version 2 of the License, or
%    (at your option) any later version.

%    This program is distributed in the hope that it will be useful,
%    but WITHOUT ANY WARRANTY; without even the implied warranty of
%    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%    GNU General Public License for more details.

%    You should have received a copy of the GNU General Public License along
%    with this program; if not, write to the Free Software Foundation, Inc.,
%    51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.

% New in version 1.2:
% - level-specific styles (thanks to Andrew Stacey)

% New in version 1.11:
% - make options compatible with standard tikz trees

% New in version 1.1:
% - sideways trees

%% These macros facilitate building up an object recursively before
%% putting it into the input stream.

\newtoks\@result
\def\@call#1#2{\let\@cont=#2\bgroup\@result={}#1}
\def\@return{\global\@result=\@result\egroup\@cont}

\def\@ifequal#1#2{\edef\testa{#1}\edef\testb{#2}\ifx\testa\testb}

%% scan a tree: this just scans a subtree and then puts it onto the
%% input stream

\def\Tree{\@call\@subtree\@Tree}
\def\@Tree{%
%\showthe\@result %debug
\ifpgfpicture % is there a test for tikzpicture?
\pgftree{\the\@result}%
\else
\tikzpicture[baseline]\pgftree{\the\@result}\endtikzpicture
\fi
}

%% scan a subtree
\newtoks\child@list
\newtoks\root@node

\def\@subtree[{%
\root@node={}%
\pgfutil@ifnextchar.{\@call\@interior\@@subtree}{\@@@subtree}}
\def\@@subtree{%
\root@node=\@result
\@@@subtree
}
\def\@@@subtree{%
\@call\@children\@@@@subtree
}
\def\@@@@subtree]{%
\child@list=\@result
\pgfutil@ifnextchar.{\@call\@interior\@@@@@subtree}{\@@@@@@subtree}}
\def\@@@@@subtree{%
%%% Check for mismatch.
\@ifequal{\the\root@node}{\pgfutil@empty}%
  \root@node=\@result
\fi
\@ifequal{\the\root@node}{\the\@result}\else
  \message{Warning: mismatched labels, \the\root@node{} and \the\@result.}%
\fi
\@@@@@@subtree
}
\def\@@@@@@subtree{%
\@ifequal{\the\root@node}{\pgfutil@empty}%
\edef\act{\noexpand\@result={%
\noexpand\subtree@hook
\noexpand\pgfsubtree{\noexpand\path coordinate (\noexpand\nodename);}{\the\child@list}}}%
\else
\edef\act{\noexpand\@result={%
\noexpand\subtree@hook
\noexpand\pgfsubtree{\the\root@node}{\the\child@list}}}%
\fi
\act
\@return}

%% scan a sequence of subtrees or leaves

\newif\ifscanned@edge

\def\@children{%
\scanned@edgefalse
\child@list{}%
\@@children}
\def\@@children{%
\pgfutil@ifnextchar]{\@result\child@list\@return}{% end of children
\pgfutil@ifnextchar\edge{% explicit edge
\ifscanned@edge
\message{Warning: more than one edge given for a single child}\let\next\@@children % ignore
\else
\scanned@edgetrue\let\next\@@@children
\fi
\@call\@edge\next}{%
% else, a real node is next
\ifscanned@edge\else % no explicit edge, supply default
\expandafter\child@list\expandafter{\the\child@list{\edge@adapter{}}}%
\fi
\scanned@edgefalse
\pgfutil@ifnextchar[{% subtree
\expandafter\child@list\expandafter{\the\child@list{\level@hook\interior@hook}}%
\@call\@subtree\@@@children}%
{% leaf
\expandafter\child@list\expandafter{\the\child@list{\level@hook\frontier@hook}}%
\@call\@leaf\@@@children}%
}}}
\def\@@@children{%
% wrap child inside curly braces
\expandafter\@result\expandafter{\expandafter{\the\@result}}%
\edef\act{\noexpand\child@list{\the\child@list \the\@result}}\act
\@@children
}

\def\@interior.{\@result{\node[alias=\nodename][every tree node,every internal node,every level \the\pgftree@level\space node/.try]}\@label}

\def\@leaf{\@call\@label\@@leaf}
\def\@@leaf{\edef\act{\noexpand\@result{%
\noexpand\subtree@hook
\noexpand\pgfsubtree{\noexpand\node[alias=\noexpand\nodename][every tree node,every leaf node,every level \noexpand\the\pgftree@level\space node/.try]\the\@result}{}}}\act\@return}

\def\@edge\edge #1;{%
\@result{\edge@adapter{#1}}%
\@return}
\def\edge@adapter#1{%
\let\tikzparentnode\parentnodename
\let\tikzchildnode\nodename
\path edge from parent #1;%
}

\def\level@hook{%
{\advance\pgftree@level by 1\relax
\xdef\@act{\noexpand\tikzset{level \the\pgftree@level/.try}}}\@act}
\def\subtree@hook{%
%\edef\act{\noexpand\tikzset{every tree node/.append code={\noexpand\tikzset{every level \the\pgftree@level+ node/.try}}}}\act
{\advance\pgftree@level by 1\relax
\xdef\@act{\noexpand\tikzset{level \the\pgftree@level+/.try}}}\@act
}
\def\interior@hook{\tikzset{interior/.try}}
\def\frontier@hook{\tikzset{frontier/.try}}

% a label is either text or PGF/TikZ code starting with \node
\def\@label{\pgfutil@ifnextchar\node{\@litlabel}{\@@label}}
\def\@@label#1 {%
\expandafter\@result\expandafter{\the\@result{#1};}%
\@return}

% try to copy \node command into \@result without stripping braces
\def\@litlabel\node{\@@litlabel}
\def\@@litlabel{\pgfutil@ifnextchar\bgroup{\@@@litlabel}{\@@@@litlabel}}
\def\@@@litlabel#1{\expandafter\@result\expandafter{\the\@result {#1}}\@@litlabel}
\def\@@@@litlabel#1;{\expandafter\@result\expandafter{\the\@result #1;}\@return}

% predefined edges

\def\tree@edge#1#2{(#1.\pgftree@parentanchor) -- (#2.\pgftree@childanchor)}

\def\roof@edge#1#2{\csname roof@edge@\leveldirection\endcsname{#1}{#2}}
\def\roof@edge@down#1#2{(#1.south) -- (#2.north west) -- (#2.north east) -- cycle}
\def\roof@edge@up#1#2{(#1.north) -- (#2.south west) -- (#2.south east) -- cycle}
\def\roof@edge@left#1#2{(#1.west) -- (#2.north east) -- (#2.south east) -- cycle}
\def\roof@edge@right#1#2{(#1.east) -- (#2.north west) -- (#2.south west) -- cycle}

%%% Options
\pgfkeysgetvalue{/tikz/level distance/.@cmd}{\orig@leveldistance}
\tikzoption{level distance}{\pgfmathsetlength\levelsep{#1}\orig@leveldistance#1\pgfeov}
\tikzoption{distance from root}{\pgfmathsetlength\levelsep{#1}\advance\levelsep by -\pgftree@depth}
\pgfkeysgetvalue{/tikz/sibling distance/.@cmd}{\orig@siblingdistance}
\tikzoption{sibling distance}{\pgfmathsetlength\subtreesep{#1}\orig@siblingdistance#1\pgfeov} % different semantics

% I don't really like this scheme
\pgfkeysgetvalue{/tikz/grow/.@cmd}{\orig@grow}
\tikzoption{grow}{\csname grow@#1\endcsname\orig@grow#1\pgfeov}
\pgfkeysgetvalue{/tikz/grow'/.@cmd}{\orig@growprime}
\tikzoption{grow'}{\csname growprime@#1\endcsname\orig@growprime#1\pgfeov}
\def\grow@up{\def\leveldirection{up}\def\siblingdirection{left}}
\def\grow@down{\def\leveldirection{down}\def\siblingdirection{right}}
\def\growprime@up{\def\leveldirection{up}\def\siblingdirection{right}}
\def\growprime@down{\def\leveldirection{down}\def\siblingdirection{left}}
\def\grow@left{\def\leveldirection{left}\def\siblingdirection{down}}
\def\grow@right{\def\leveldirection{right}\def\siblingdirection{up}}
\def\growprime@left{\def\leveldirection{left}\def\siblingdirection{up}}
\def\growprime@right{\def\leveldirection{right}\def\siblingdirection{down}}

% defaults appropriate for linguistic trees
\def\tikz@edge@to@parent@path{\tree@edge{\tikzparentnode}{\tikzchildnode}}
\tikzset{every tree node/.style={anchor=base}}
\tikzset{every leaf node/.style={}}
\tikzset{every internal node/.style={}}

% predefined roof style
\tikzset{roof/.style={edge from parent path=\roof@edge{\tikzparentnode}{\tikzchildnode}}}

